Planning the Future of U.S. Particle Physics (Snowmass 2013): Chapter 1: Summary

These reports present the results of the 2013 Community Summer Study of the APS Division of Particles and Fields ("Snowmass 2013") on the future program of particle physics in the U.S. Chapter 1 contains the Executive Summary and the summaries of the reports of the nine working groups.

==> Frontiers/Conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}


Conclusions go here.

==> Frontiers/IF4page.tex <==


\section{Intensity Frontier}
\label{sec:IF}

All frontiers of high energy physics aim to discover and understand the constituents of matter and their interactions at the highest energies, at the shortest distances, and at the earliest times in the Universe. The Standard Model fails to explain all observed phenomena: new interactions and yet unseen particles must exist. They may manifest themselves either directly, as new particles, or by causing Standard Model reactions to differ from often very precise predictions. The Intensity Frontier explores these fundamental questions by searching for new physics in processes extremely rare or those forbidden in the Standard Model. This requires the greatest possible beam intensities, as well as massive ultra-sensitive detectors. Many of these experiments are sensitive to new physics at higher mass scales, or weaker interaction strengths, than those directly accessible at high-energy colliders, thus providing opportunities for paradigm-changing new discoveries complementary to Energy and Cosmic Frontier experiments.

The range of experiments encompassing the Intensity Frontier is broad and diverse. Intense beams of neutrinos aimed over long distances at very large detectors will explore the neutrino mass hierarchy, search for CP violation and non-standard interactions, and increase sensitivity to proton decay. Multi-ton-scale detectors will determine whether neutrinos are their own antiparticles. Intense beams of electrons will enable searches for hidden-sector particles that may mediate dark matter interactions. Extremely rare muon and tau decay experiments will search for violation of charged lepton quantum numbers. Measurements of intrinsic lepton properties, such as electric and magnetic dipole moments are another promising thrust. Rare and CP-violating decays of bottom, charm, and strange particles, measured with unprecedented precision, will be important to unravel the new physics underlying discoveries at the LHC. In any new physics scenario, Intensity Frontier experiments with sensitivities to very high mass scales will be a primary tool for exploration.

At Snowmass, the intensity frontier program was defined in terms of six areas that formed the basis of working groups:  experiments that probe ($i$) Neutrinos, ($ii$) Baryon Number Violation, ($iii$) Charged Leptons, ($iv$) Quark Flavor Physics, ($v$) Nucleons, Nuclei, and Atoms, and ($vi$)  New Light, Weakly-coupled Particles,.  

The working group reports provide a clear overview of the science program within each area of the intensity frontier.  The discovery opportunities are presented for facilities that will be available this decade or come on line during the next decade.  Here, we briefly summarize the findings from each working group. 

\noindent{\bf Neutrinos:} 
Decades of experimental and observational scrutiny have revealed less than a handful of phenomena outside the standard model: the dark energy and dark matter puzzles, and the existence of non-zero neutrino masses.
The existence of non-zero neutrino mass represents one of the few experimental pointers towards a new description.     
While many experiments continue to look for other new phenomena and deviations from standard model predictions, it is clear that continued detailed study of the neutrino sector is of the utmost importance.    
 
Compared to the other fermions, the elusive nature of the neutrino has made it extremely difficult to study in detail.    In spite of the challenges, neutrino physics
has been tremendously successful over the past two decades.  From almost 
complete lack of knowledge about neutrino mass and mixing twenty years ago,
we now have a robust, simple, three-flavor paradigm, describing most of the data.  However, key questions in the three-flavor sector remain -- we do not know the mass ordering, nor whether neutrinos violate CP symmetry, nor whether the neutrino is its own
antiparticle, and we
have only just began to test the three-flavor paradigm. A precision neutrino oscillation program is required to carry out such measurements.
Furthermore, some experiments have uncovered intriguing anomalies that merit additional study, and could lead to the discovery of beyond-the-standard-model states or interactions.
Advances in detector technology and analytical techniques needed for the next generation of neutrino experiments are well underway.  
We have clear experimental paths forward for building on our success, both for precision testing of the three-flavor paradigm, and for exploration of anomalies.
 
The next decade promises significant experimental progress around the world.  In the search for neutrinoless double-beta decay, a number of experiments rely on complementary isotopes and experimental techniques.  
The next generation of 100-kg-class neutrinoless double-beta-decay search experiments should have sensitivity to effective masses in the 100~meV range; beyond that, there are opportunities for multi-ton-class experiments that will reach sub 10~meV effective mass sensitivity, pushing below the inverted hierarchy region.  The next generation of tritium-beta-decay experiments will directly probe neutrino masses a factor of 10 smaller the best current bounds; innovative new ideas may help to go beyond these sensitivities.  

%Current experiments will continue to take data, and
%there is vigorous worldwide activity towards planning for large-scale next-generation long-baseline efforts.  There are exciting opportunities for the US to take leadership in this arena with LBNE, and beyond that, Project X, for increased neutrino intensity at several beam energies.  There are additional opportunities for international collaboration.
%Given the challenges associated with precision measurements in the neutrino sector, complementary baselines, sources and detector techniques will be needed to help further understand the nature of CP violation in the neutrino sector.  Smaller experiments will also help address some of the remaining anomalies and hints for new physics beyond the three-flavor paradigm.
% 

The neutrino mass hierarchy can be unambigously resolved using accelerator neutrino oscillation experiments with
baselines around 1000~km (or larger) and detector masses of order tens of kilotons.  
Precision
measurements of atmospheric neutrino oscillations with megaton scale
underground detectors can also resolve the mass hierarchy.  
The discovery
of a non-zero $\theta_{13}$ enables long-baseline neutrino experiments to
search for leptonic CP violation in appearance experiments. 
The search for CP violation in the neutrino sector is a top priority for particle physics
efforts worldwide,
and a vigorous planning for the next generation large
scale neutrino oscillation experiment is underway internationally.
Regardless of the experimental approach, high-power proton beams
(greater than 1~MW) coupled with massive  detectors (order 100~kton), are needed to study CP violation in neutrino oscillations. 
%Experiments with baselines around 1000~km coupled
%with wide-band beams that cover a large region of the neutrino oscillation
%space offer the best sensitivity to CP violation and high precision
%determination of the CP phase $\delta$ is possible with exposures under 1000. 
The U.S., with the Long-Baseline Neutrino Experiment (LBNE) and a future multi-megawatt beam from Project
X at Fermilab, is uniquely positioned to lead an international campaign to measure CP violation
and push the limits of the three-flavor paradigm. 
An underground location for a far detector significantly enhances the physics reach.  LBNE represents a vibrant global
program with the U.S. as host.

Given the challenges associated
with precision measurements in the neutrino sector, complementary baselines, sources and detector techniques will be required to piece together a sharp picture. 
New accelerator technologies, such as
neutrino factories and cyclotron-based-sources, may in the long term
take measurements to the next level. Smaller
experiments will also play a key role in addressing some of the remaining
anomalies and hints for physics beyond the three-neutrino paradigm, and study neutrino--matter interactions in detail.
 
The diversity of physics topics that can be probed through the neutrino sector is very significant, and the interplay between neutrino physics and other fields is rich.   Neutrinos can and will provide important information on structure formation in the early universe, Earth, solar and supernova physics, nuclear properties, and rare decays of charged leptons and hadrons.   In other words, the neutrino sector sits at the nexus of the worldwide effort in energy, intensity and cosmic frontier physics.
 
The unique physics potential and technological advancements have conspired to produce a fertile environment for new ideas for improved measurements and new techniques, as well as both direct and spin-off applications.   This provides an important training ground for the next generation of scientists and engineers, and exciting ideas to share with the public.


\noindent{\bf Baryon Number Violation:}
The stability of ordinary matter is attributed to the conservation of baryon number.
Within the Standard Model protons are stable, as baryon number is assumed to be conserved.  However, baryon number is not a fundamental symmetry of the SM and is not conserved in many of its extensions.  In particular, baryon number violation is an essential ingredient for the creation of the observed asymmetry of matter over anti-matter in the universe.
Grand Unified Theories (GUTs) predict that the proton decays with a lifetime in excess of $10^{30}$ years, with the decay being mediated at scales of order $10^{16}$ GeV.  Two important decay channels in GUTs are $p\to e^+\pi^0$ and $\bar\nu K^+$, with several other modes also being possible.  The current limits on the proton lifetime in these two channels are $10^{34}$ years and $4\times 10^{33}$ years, respectively, which is a factor of five to 10 below predictions in well-motivated GUT models.

The search for proton decay is carried out in large underground detectors – large to amass enough protons and underground to reduce backgrounds.  Large neutrino oscillation detectors are ideal for this task, and proton decay is an important piece of their physics portfolio.  The current largest underground neutrino experiment is a tens of ktons water Cherenkov detector. Future underground neutrino experiments with projected target masses of 34 ktons of liquid Ar or 200 - 500 ktons of water can measure lifetimes on the order of GUT expectations with exposures of roughly 10 years. Typically, a 5.6 Megaton-year exposure could reach a sensitivity of $\tau(p\to  e^+ pi^0) < 10^{35}$ years and $\tau(p\to\bar\nu K^+<2.5\times 10^{34}$ years.  

Neutron-antineutron oscillations would violate baryon number by two units and are searched for with a beam of free neutrons where one neutron transforms into an antineutron and annihilates in a distant detector.  A new experiment at Project X at Fermilab uses free neutrons from a 1 MW spallation target and could improve existing constraints by 4 orders of magnitude.

\noindent{\bf Charged Leptons:}
The physics potential of the charged lepton experimental program is significant with discovery opportunities in experiments
being conducted this decade and in even more sensitive experiments possible with future facilities such as Project X at Fermilab.
Extremely sensitive searches for rare decays of muons and tau leptons, together with precision measurements of their properties, will either elucidate the scale and dynamics of flavor generation, or limit the scale of flavor generation to well above $10^4$ TeV.
Any indication of charged Lepton Flavor Violation (CLFV) would be an indisputable discovery of new physics. Precision measurments of Lepton Flavor Conserving (LFC) processes can be used to verify predictions of the SM and look for signs of new physics.

The experimental program consists of a large and diverse set of opportunities and includes multi-purpose experiments that utilize the large tau production rates at high-luminosity $B$ factories, as well as highly optimized single-purpose experiments that explore muon transitions.

Significant advances in studying CLFV in the muon sector can be achieved this decade.  For the rare decay $\mu\to e\gamma$,  MEG at the Paul Scherrer Institute can reach a sensitivity of $10^{-13}$.   For $\mu\to 3e$, two new experiments, mu3e at PSI and MuSIC at Osaka University, have plans to improve the current sensitivity by approximately four orders of magnitude.  Current limits for $\mu N\to e N$ conversion are obtained at experiments at PSI (with Ti and Au nuclei) at the level of $10^{-12}-10^{-13}$.  DeeMe at J-PARC plans to improve these bounds by two orders of magnitude.  Later in this decade, COMET at J-PARC and Mu2e at Fermilab could improve the existing search reach by four orders of magnitude.  This would bring the sensitivity to such conversions to $\sim 10^{-17}$ by the end of this decade, which is a level where  signals from supersymmetric grand unified models are expected to lie.  If no signal is observed, this would set constraints on CLFV physics at the scale of $10^4$ TeV.  Future experiments beyond these are being considered in conjunction with more intense muon beams, which in return require more intense proton beams that could be provided by upgraded facilities at J-PARC or Project-X at Fermilab.

The classic example for studying LFC processes with muons is the measurement of the muon’s magnetic moment, which is predicted very precisely (five-loop level) in the SM. New physics contributes via radiative corrections, and would yield an anomalous value of $g\neq 2$.  The present level of sensitivity was obtained by the E821 experiment at Brookhaven National Laboratory, with a difference between the measurement and the SM theoretical prediction of $(287\pm 80) \times 10^{-11}$,  a $3.6\sigma$ deviation from the SM value.  A new experiment, E989, will employ the E821 muon storage ring at Fermilab and will use the same experimental techniques. It aims to increase the statistics by a factor of 20 while keeping the other uncertainties at the same level of 0.1ppm, resulting in an overall reduction in the experimental error by a factor of roughly four. An alternate approach, being developed at J-PARC using lower-energy muons,  is expected to have the same statistical uncertainty as E989 at Fermilab but with very different systematics.  In addition, the lattice gauge community is undertaking computations to reduce the theoretical error inherent in this process.

The important observables in $\tau$ decays are CLFV decays, polarized decays, the electric dipole moment, and the anomalous magnetic dipole moment.  New physics effects usually scale as a function of the lepton mass, and hence $\tau$ observables can be very sensitive to new contributions.  The large $\tau$ production rates possible at the future SuperKEKb facility in Japan could reach the level of $10^{-9-10}$ in CLFV branching fractions, which represents an order of magnitude improvement over current results from BABAR and Belle.

The charged lepton sector has significant potential to reveal more information on the fundamental principles of Nature, and the US has the opportunity to play a leading role with facilities planned for this decade.


\noindent{\bf Quark Flavor Physics:}
The study of strange, charm, and bottom quark systems has a long and rich history in particle physics as measurements of rare processes in the flavor sector have led to startling revelations and played a critical role in the development of the Standard Model.  The constraints on physics beyond the SM from flavor physics considerations are powerful.  
While the current quark flavor data set is in agreement with SM expectations, new corrections to the SM at the level of tens of percent are still allowed.  Contributions to flavor processes from many theories beyond the SM arise at this level, and thus more precise measurements may observe new physics.  In particular, if new massive states are observed at the CERN Large Hadron Collider (LHC), then detailed measurements of the quark flavor sector will be necessary to determine the underlying theory and its flavor structure.  If such states are not discovered in high energy collisions, then precision quark flavor experiments, with their ability to probe mass scales far beyond the reach of the LHC, provide the best opportunity to set the next energy scale to explore. Depending on the strength of new physics interactions, this program already indicates that the new physics scale is above $1-10^5$ TeV, and proposed experiments can probe even further.  Continued investigations of the quark flavor sector are thus strongly motivated.

A well-planned program of flavor physics experiments has the potential to continue this history of advances.  Such a program exists worldwide with the LHCb experiment at the LHC, an upgraded SuperKEKb facility in Japan, BESIII in China, and future rare kaon decay experiments at CERN, J-PARC and potentially Fermilab.  These facilities have the potential to carry out a rich multi-purpose program in the strange, charm, and bottom sector and perform numerous crucial measurements of rare decays and $CP$-violating observables. In particular, the proposed experiment ORKA at the Fermilab Main Injector would probe rare Kaon decays to unprecedented precision and would retain the U.S. capability to perform quark flavor experiments.  Longer term, Project X at Fermilab could become the dominant facility in the world for rare Kaon decays. The expected sensitivities for these future programs are detailed in the full report, and at are the level which could discover new physics.  It is important to note that these results are not predicated on future theoretical progress, although theoretical advancements will strengthen the program by increasing the set of meaningful observables.  
U.S. contributions and support for quark flavor experiments are necessary in order for the U.S. HEP program to have the breadth to assure meaningful participation in future discoveries.


\noindent{\bf Nucleons, Nuclei, and Atoms:}
The use of nucleons, nuclei, and atoms as laboratories for the study of fundamental interactions is entering a
new era.  Observables involving these systems
have sensitivity to physics beyond the Standard Model and provide important tests of vital symmetries.  
Measurements of electric dipole moments (EDMs), weak decays of light hadrons, weak neutral currents, and atomic parity violation are particularly well-suited in this regard.  

Observation of an EDM would be a direct signature of both parity and time-reversal symmetry violation, and probes the physics of $CP$ violation which necessarily accompanies $T$ violation under the $CPT$ theorem.  The SM prediction (via multi-loop contributions) for the EDM of the electron, neutron, and nucleus is $10^{-38}\,, 10^{-31}$, and $10^{-33}$ {\it e}$\cdot$cm, respectively.  EDM measurements are challenging
and the present experimental sensitivity is at the level of $10^{-27}\,, 3\times 10^{-26}$, and $3\times 10^{-29}$ {\it e}$\cdot$cm for the electron, nucleon, and $^{199}$Hg nucleus, respectively. Experiments searching for the electron EDM typically use the polar molecules YbF and ThO and ultimately expect to reach a level of $3 \times 10^{-31}$ {\it e}$\cdot$cm.  Several experiments searching for the neutron EDM are planned or under way and are expected to reach a sensitivity of $5\times 10^{-28}$ {\it e}$\cdot$cm, which constitutes a factor of 100 improvement over current limits.  For atoms, future experiments using Hg , radon and radium expect sensitivity at the level $10^{-32}$ {\it e}$\cdot$cm.  This would require upgraded facilities such as FRIB at Michigan State University or Project X at Fermilab.  The expected sensitivity of these future programs is at the level where signals are predicted to appear in several theories beyond the SM.

The weak decays of light hadrons provide precision input to the SM and are a sensitive test of new interactions. The ratio of decay channels $e\nu/\mu\nu$ for pions and kaons affords an accurate test of lepton universality and can probe new physics up to 1000 TeV.  For pions, experiments under way at TRIUMF and PSI will improve the measurement error by a factor of five and probe the SM to the level of 0.1\%. Neutron beta decay provides the most accurate determination of the CKM element $V_{ud}$, enabling strong tests of CKM unitarity and constraining new physics up to scales of $\sim 10$ TeV.  Several programs are underway to measure observables of the neutron lifetime and decay asymmetries with improved precision.
Measurements of parity-violating asymmetries in fixed-target scattering with polarized electrons allows for a precision determination of the weak mixing angle at low values of momentum transfer, which in turn constrains new parity-violating effects up to $2-3$ TeV.  Improved polarized Moller scattering experiments at upgraded JLab facilities expect to determine the weak mixing angle to an accuracy of $0.1\%$, which is comparable to measurements at the $Z$-pole.  Parity violation in atomic transitions also yields valuable measurements of the weak mixing angle and new techniques requiring intense sources are being developed and Project X at Fermilab that would provide more rare isotopes for this program than any other facility. 

\noindent{\bf New Light, Weakly Coupled Particles:}
New light particles that couple very weakly to the SM fields are a common feature of extensions beyond the SM.  They are motivated by both theoretical and observational considerations, including the strong $CP$ problem and the nature of dark matter and dark energy.  Examples of such particles include axions, hidden-sector photons, milli-charged particles, and chameleons.  These hidden-sector particles typically couple to the photon via a mixing effect, so that they only interact very weakly with the photon.  Intense sources are hence required to produce them at rates sufficient to enable their discovery.
The parameters relevant for searches of such hidden-sector particles are their mass and coupling strength to the photon.  A variety of observations constrain part of this parameter space, but much territory is still open for exploration.  In particular, regions that are consistent with dark matter observations and areas that offer an explanation for the present result on the anomalous magnetic moment of the muon have yet to be probed.  The current constraints arise from astronomical observations, cosmological arguments, and a variety of laser, heavy flavor, and fixed-target experiments.

There is much activity on the experimental front, and several laboratory experiments are either in progress or proposed.  Two ADMX-type microwave cavity searches for axions will be under way soon in the US, but require further developments to increase their mass reach.  The light-shining-through-walls technique, where photons are injected against an opaque barrier, continues to explore open regions of parameter space.  More advanced technology is needed to make progress in the mid-term.  Axion helioscope searches were first carried out using borrowed magnets, and now require a custom-built magnet to improve sensitivity.  Collider searches for hidden-sector particles can be performed via the reaction $e^+e^-\to\gamma\ell^+\ell^-$ at high luminosity $B$ factories or in the decays of gauge bosons at the LHC.  Fixed-target experiments using both electron and proton beams are a promising place to search for hidden-sector particles.  The electron beam experiments APEX at Jefferson Laboratory  and A1 at the University of Mainz have recently performed short test runs and have plans for more extensive runs this decade.  HPS has been approved by JLab and will run after the 12 GeV upgrade is installed at CEBAF.  DarkLight proposes to use the free-electron laser beam at JLab.  Proton fixed-target experiments have the potential to explore regions of parameter space that cannot be probed by any other technique.  Neutrino experiments, such as MiniBooNe, can widen the search to smaller couplings. The intense proton source at Project X could also provide a powerful extension to the search reach.   
Impressively large regions of parameter space are currently unexplored and are ripe for the discovery of light, weakly coupled particles.


\noindent{\bf Summary:}
The above program exhibits the broad spectrum of science opportunities attainable at the intensity frontier.  While each subfield is at a different stage of maturity in terms of testing the SM, the proposed experiments in each area are poised to have major impact.  The programs involving transitions of heavy quarks, charged leptons, and nucleons, nuclei, and atoms are advanced, with the most precise SM predictions and a well-developed experimental effort that has spanned decades.  In this case, the next level of experimental precision would reach the point where effects of new TeV-scale interactions are expected to be observable.  More sensitive searches for proton decay and new light, weakly coupled particles can cover a large range of parameter space that is consistent with Grand Unified Theories and cosmological observations.  Neutrino physics is just begining the era of precision measurements where it is possible to probe basic neutrino properties and answer principal questions.  Neutrino physics therefore holds great promise for discovery. 

Such an extensive program is necessary to address the unresolved fundamental questions about Nature.  The knowledge we seek cannot be gained by a single experiment or on a single frontier, but rather from the combination of results from many distinct approaches working together in concert.  The full report provides a reference for the captivating science that can be carried out at the intensity frontier this decade and next.  The intensity frontier program has the potential to make discoveries that change paradigms and alter our view of the universe.  

\end{document}





==> tcilcomm.tex <==
% Macros used for TCI styles released with Scientific Word 1.1.
%Copyright (C) 1992-93 TCI Software Research, Inc.
\typeout{TCILCOMM Macros for TCI styles <08 Apr 93>.}
%
% Revisions:
% 08 Apr 93 - GP change line length to under 80 characters
% 30 Mar 92 - AO added \setmoremathsizes and hooks to, e.g. \@xpt,
%             for support of bold Greek
%
%%ltg added this to try to get 12pt to come through
%\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
%%end ltg

\def\@ptoptions{%
 \let\@elt\relax\@for\@tempa:=\@optionlist\do{%
  \expandafter\let\expandafter\@tempb\csname ds@\@tempa\endcsname
  \expandafter\let\expandafter\@tempc\csname ds@11pt\endcsname
  \ifx\@tempb\@tempc\else
   \expandafter\let\expandafter\@tempc\csname ds@12pt\endcsname
   \ifx\@tempb\@tempc\else\let\@tempb\relax\fi
   \fi
  \@tempb
  }%
 }%
%
% read in style file, but only process the pt size options
%
\def\@ptoptinput#1{%
 \let\@save@optionlist\@optionlist
 \let\@save@options\@options
 \let\@options\@ptoptions
 %
 \input #1
 %
 \let\@optionlist\@save@optionlist
 \let\@options\@save@options
 }%
%
% the <21 Feb 92> version of letter.sty requires:
\ifx\undefined\reset@font
 \def\reset@font{}%
 \fi
%
% Change LaTeX
%
% Add command to append tokens
\newtoks\@temptokenb
\long\def\appdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokena\the\@temptokenb}%
 }%
\long\def\prepdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokenb\the\@temptokena}%
 }%
% Discard contents of \box\@cclv at beginning of document
\appdef\document{{\output{\setbox\z@\box\@cclv}\endgraf\null\eject}}%
% Fix mark register expansion
\def\leftmark{\expandafter\@leftmark\botmark{}{}{}\@nil}%
\def\rightmark{\expandafter\@rightmark\firstmark{}{}{}\@nil}%
\def\@leftmark#1#2#3\@nil{#1}%
\def\@rightmark#1#2#3\@nil{#2}%
%
%\show\raggedright
\newskip\raggedglue
\raggedglue\z@ plus20\p@ minus\z@
\def\raggedright{%
 \let\\=\@centercr\@rightskip\raggedglue\rightskip
 \@rightskip\leftskip\z@\parindent\z@
 }%
%
\def\@centercr{%
 \ifhmode\unskip\else\@badcrerr\fi\@@par
 \@ifstar{\penalty\@M\@xcentercr}{\@xcentercr}%
 }%
%
\def\traceoutput{\tracingoutput2\showboxbreadth\maxdimen
 \showboxdepth\maxdimen}%
%
\newcount\@hour\newcount\@minute\chardef\@x10\chardef\@xv60
\def\@time{%
  \@minute\time\@hour\@minute\divide\@hour\@xv
  \ifnum\@hour<\@x 0\fi\the\@hour:%
  \multiply\@hour\@xv\advance\@minute-\@hour
  \ifnum\@minute<\@x 0\fi\the\@minute
  }%
%
% change \@array to allow \par to mean something within its scope
%
\def\@array [#1]#2{%
 \setbox\@arstrutbox\hbox{\vrule height\arraystretch\ht
  \strutbox depth\arraystretch\dp\strutbox width\z@}%
 \@mkpream{#2}%
 \edef\@preamble{\halign\noexpand\@halignto\bgroup\tabskip
  \z@\@arstrut\@preamble\tabskip\z@\cr}%
 \let\@startpbox\@@startpbox\let\@endpbox\@@endpbox
 \if#1t\vtop\else\if#1b\vbox\else\vcenter\fi\fi
 \bgroup
  %\let\par\relax
  \let\@sharp##
  \let\protect\relax
  \lineskip\z@\baselineskip\z@
  \@preamble
 }%
%
% Expands to hex digit corresponding to the value of the argument
%
\def\hexnumber@#1{\ifnum#1<10 \number#1\else
 \ifnum#1=10 A\else\ifnum#1=11 B\else\ifnum#1=12 C\else
 \ifnum#1=13 D\else\ifnum#1=14 E\else\ifnum#1=15 F\fi\fi\fi\fi\fi\fi\fi}%
%
% define command to set more math sizes.
% Styles like Greekbf will hook in here.
%
\def\setmoremathsizes#1#2#3{}%
%
% define size switch addenda
%  Note: these choices agree with those in lfonts.tex, even if incorrect.
%
\prepdef\@vpt{\setmoremathsizes{fiv}{fiv}{fiv}}%
\prepdef\@vipt{\setmoremathsizes{six}{six}{six}}%
\prepdef\@viipt{\setmoremathsizes{sev}{fiv}{fiv}}%
\prepdef\@viiipt{\setmoremathsizes{egt}{six}{fiv}}%
\prepdef\@ixpt{\setmoremathsizes{nin}{six}{fiv}}%
\prepdef\@xpt{\setmoremathsizes{ten}{sev}{fiv}}%
\prepdef\@xipt{\setmoremathsizes{elv}{egt}{six}}%
\prepdef\@xiipt{\setmoremathsizes{twl}{egt}{six}}%
\prepdef\@xivpt{\setmoremathsizes{frtn}{ten}{sev}}%
\prepdef\@xviipt{\setmoremathsizes{svtn}{twl}{ten}}%
\prepdef\@xxpt{\setmoremathsizes{twty}{frtn}{twl}}%
\prepdef\@xxvpt{\setmoremathsizes{twty}{twty}{svtn}}%
%
% The \newfield command defines (like \newenvironment) a user syntax:
%
%   \newfield{foo}
%
% lets you write
%
%   \begin{foo}...\end{foo}
%
% but differs from \newenvironment in that TeX parses the entire content
% of the field and stores it in a macro \the@foo, and then executes \@do@foo.
%
% This means that the content of the field is actually more like an argument
% than the content of an environment. So \verb will not necessarily work
% within a field, and neither will \index. Caveat emptor.
%
% The default procedure for a field is to process its argument within a
% group.  If you want a field to simply store its data away, define its
% procedure to be synonymous with \@empty, as illustrated below.
%
\long\def\@readenvir#1#2\end{%
 \appdef\envirsofar{#2}%
 \@ifnextchar\bgroup{\@checkenvir{#1}}{\@envirenderr}%
 }%
%
\def\@envirenderr{%
 \@latexerr{\string\end\space not followed by environment name}\@eha
 }%
%
\def\@checkenvir#1#2{%
 \def\@tempa{#1}\def\@tempb{#2}%
 \ifx\@tempa\@tempb
  \ifx\envirsofar\@blankspace\let\envirsofar\@empty\fi
  \expandafter\let\csname the@#1\endcsname\envirsofar
  \def\@tempa{\csname @do@#1\endcsname}%
  \else
  \appdef\envirsofar{\end{#2}}%
  \def\@tempa{\@readenvir{#1}}%
  \fi
 \@tempa
 }%
%
\def\newfield#1#2{%
 \expandafter\@ifdefinable\csname#1\endcsname{%
  \expandafter\def\csname#1\endcsname{%
   \endgroup\let\envirsofar\@empty\@readenvir{#1}%
   }%
  \expandafter\let\csname the@#1\endcsname\@empty
  \expandafter\ifx\csname @do@#1\endcsname\relax
   \expandafter\def\csname @do@#1\endcsname{{\csname the@#1\endcsname}}%
   \fi
  }%
 }%
%
\def\@blankspace{ }% SciWord's nil field
%
\def\letparBL{\def\par{\\}}%
\def\letparSP{\def\par{\ }}%
\def\letparQD{\def\par{\quad}}%
\def\letparSL{\def\par{\hbox to1em{\hfil/\hfil}}}%
%
% When \par is processed in the page head, gobble up the rest of the
% argument.
\def\@gobblepar#1\@empty{}%
%
% Physical page size after trim
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\botmargin
\newdimen\marginpartotal
%
\def\adjustpagemargin{% adjust \oddsidemargin by \marginpartotal
 \marginpartotal\marginparwidth\advance\marginpartotal\marginparsep
 \advance\oddsidemargin\marginpartotal
 }%
%
\def\settextheight{% calculate textheight constrained by:
 \textheight\trimheight
 \advance\textheight-\topmargin
 \advance\textheight-\headheight
 \advance\textheight-\headsep
 \advance\textheight-\footskip
 \advance\textheight-\botmargin
 }%
%
\def\vcenterpagemargin{% calculate \topmargin constrained by:
 \topmargin\trimheight
 \advance\topmargin-\textheight
 \advance\topmargin-\headheight
 \advance\topmargin-\headsep
 \advance\topmargin-\footskip
 \divide\topmargin\tw@\botmargin\topmargin
 }%
%
\def\centerpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \divide\oddsidemargin\tw@
 \evensidemargin\oddsidemargin
 \adjustpagemargin
 }%
%
\def\leftpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \advance\oddsidemargin-\evensidemargin
 \adjustpagemargin
 }%

